Coverage Sampling Planner for UAV-enabled Environmental Exploration and Field Mapping

Unmanned Aerial Vehicles (UAVs) have been implemented for environmental monitoring by using their capabilities of mobile sensing, autonomous navigation, and remote operation. However, in real-world applications, the limitations of on-board resources (e.g., power supply) of UAVs will constrain the coverage of the monitored area and the number of the acquired samples, which will hinder the performance of field estimation and mapping. Therefore, the issue of constrained resources calls for an efficient sampling planner to schedule UAV-based sensing tasks in environmental monitoring. This paper presents a mission planner of coverage sampling and path planning for a UAV-enabled mobile sensor to effectively explore and map an unknown environment that is modeled as a random field. The proposed planner can generate a coverage path with an optimal coverage density for exploratory sampling, and the associated energy cost is subjected to a power supply constraint. The performance of the developed framework is evaluated and compared with the existing state-of-the-art algorithms, using a real-world dataset that is collected from an environmental monitoring program as well as physical field experiments. The experimental results illustrate the reliability and accuracy of the presented coverage sampling planner in a prior survey for environmental exploration and field mapping.

==> Figures/Fig2.tex <==
\begin{figure}[h]
	\centering
    \subfigure{
    \includegraphics[height=5.5cm]{Fig2.pdf}}
    \caption{Edge candidates and ACC decomposition. The bold black lines denote the ACC contours. The dashed blue lines between the neibouring SLoIs denote the edge candidates.}
    \label{fig: edge candidates}
\end{figure}

==> Figures/Fig7.tex <==
   \begin{figure}[!b]
      \centering
      \includegraphics[height = 5cm]{Figure7/Fig7.eps}
      \caption{Relationships between cell size and number of SLoIs, and total length.} \label{fig:7} 
   \end{figure}

==> Figures/Fig8.tex <==
\begin{figure*}[!t]
    \centering
    % \framebox{\parbox{3.2in}{}}}
          %\subfigure[Searching Time (brute-force).]{\label{fig:8a}  
      %\includegraphics[height = 4.8cm]{Figure8/Fig8_a.eps}} \ \
        %        \subfigure[Planning Time (brute-force).]{\label{fig:8b}  
      %\includegraphics[height = 4.8cm]{Figure8/Fig8_b.eps}} \ \
                %\subfigure[Total Time (brute-force).]{\label{fig:8c}  
      %\includegraphics[height = 4.8cm]{Figure8/Fig8_c.eps}} \\
         %\ \
                \subfigure[Searching Time (binary).]{\label{fig:8d}  
      \includegraphics[height = 4.8cm]{Figure8/Fig8_d.eps}} \ \
                      \subfigure[Planning Time (binary).]{\label{fig:8e}  
      \includegraphics[height = 4.8cm]{Figure8/Fig8_e.eps}} \ \
                      \subfigure[Total Time (binary).]{\label{fig:8f}  
      \includegraphics[height = 4.8cm]{Figure8/Fig8_f.eps}} \ \
    
  \caption{Algorithm performance related to computational efficiency.}
  \label{fig:8}
  \end{figure*} 

==> Table/Table2-backup.tex <==
\begin{table}[htbp]
  \caption{Algorithm Performance on Computational Efficiency}\label{tbl: Algorithm Performance on Sampling Path Planning Approaches}
    \centering
    \begin{tabular}{ | p{0.9cm} | p{1.5cm} || p{1.1cm} | p{1cm} | p{1.1cm} | }
      \hline
      \textbf{Energy Budget} & \centering \textbf{Algorithm} & \textbf{Searching Time } & \textbf{Planning Time } & \textbf{Total Time }\\
      (km) & & (s) & (s) & (s)  \\
      \hline \hline
      & \text{SGSTC} & 39.47 & 0.98 & 40.45
      \\
      & \text{DMPP} & 106.50 & 0.71 & 107.21
      \\
      \centering 250 & \text{RSTSP} & 4277.41 & 2.85 & 4280.26
      \\
      & \text{HGSTC} & 34.75 & 0.77 & 35.52
      \\
      & \text{HGC} & 34.87 & 0.24 & \cellcolor[gray]{.8} 35.11
      \\
      & \text{HGC (binary)} & 2.59 & 0.27 & 2.86
      \\ \hline \hline
      & \text{SGSTC} & 40.09 & 1.05 & 41.14
      \\
      & \text{DMPP} & 116.27 & 0.77 & 117.04
      \\
      \centering 350 & \text{RSTSP} & 4278.55  & 3.09 & 4281.64
      \\
      & \text{HGSTC} & 35.73 & 0.79 & 36.52
      \\
      & \text{HGC} & 34.88 & 0.29 & \cellcolor[gray]{.8} 35.17 
      \\
      & \text{HGC (binary)} & 1.89 & 0.31 & 2.20
      \\ \hline \hline
      & \text{SGSTC} & 39.68 & 1.23 & 40.91
      \\
      & \text{DMPP} & 120.84 & 1.06 & 121.97
      \\
      \centering 450 & \text{RSTSP} & 4282.62 & 4.18 & 4286.80
      \\
      & \text{HGSTC} & 35.26 & 1.05 & 36.31
      \\
      & \text{HGC} & 35.69 & 0.38 & \cellcolor[gray]{.8} 36.07
      \\
      & \text{HGC (binary)} & 2.64 & 0.37 & 3.01
      \\ \hline
      %%%%%%%%%%%%% end 6th row
    \end{tabular}
  \end{table}


==> Table/Table2.tex <==
\begin{table*}[t!]
  \caption{Algorithm Performance on Computational Efficiency}\label{tbl: Algorithm Performance on Sampling Path Planning Approaches}
    \centering
    \begin{tabular}{ | p{1cm} | p{1.1cm} || p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} |}
      \hline
      \centering
      \textbf{Energy Budget} & \centering \textbf{Processing Time} & \multicolumn{2}{c|}{\textbf{SGSTC}} & \multicolumn{2}{c|}{\textbf{DMPP}} & \multicolumn{2}{c|}{\textbf{HGTSP}} & \multicolumn{2}{c|}{\textbf{HGSP}} & \multicolumn{2}{c|}{\textbf{HGC}}
      \\
      \hline
      \centering
      $b$ (km) & (s) & Brute-force & Binary &  Brute-force & Binary &  Brute-force & Binary & Brute-force & Binary & Brute-force & Binary \\ \hline \hline
      \centering 400 & Searching & 1.36 & 6.5 & 5.5 & 5.7 & N/A & 4.8 & 4.6 & 4.8 & 4.6 & 4.8 \\
      & Planning & 0.82 & 1.7330 & 2.0412 & 2.5893 & N/A & 1.5776 & 1.8274 & 1.6062 & 1.8274 & 1.6062 \\
      & Total & 2.18 & & & & N/A & & & & &
      \\ \hline
      \centering 500 & Searching & 4.5 & 4.5 & 4.7 & 4.9 & N/A & 3.7 & 3.7 & 3.7 & 3.7 & 3.7 \\
      & Planning & 2.4891 & 2.4891 & 1.8367 & 1.8225 & N/A & 1.4626 & 1.4626 & 1.4626 & 1.4626 & 1.4626 \\
      & Total & & & & & N/A & & & & &
      \\ \hline
      \centering 600 & Searching & 3.8 & 4.1 & 4.2 & 4.3 & N/A & 3.1 & 3.1 & 3.2 & 3.1 & 3.2 \\
      & Planning & 1.4565 & 2.0527 & 1.9664 & 1.6368 & N/A & 1.2319 & 1.2319 & 1.2548 & 1.2319 & 1.2548 \\
      & Total & & & & & N/A & & & & &
      \\ \hline
      \centering 700 & Searching & 3.6 & 3.8 & 3.7 & 3.7 & N/A & N/A & 2.9 & 3 & 2.9 & 3 \\
      & Planning & 1.3357 & 1.4565 & 1.4757 & 1.4757 & N/A & N/A & 1.2120 & 1.2448 & 1.2120 & 1.2448 \\
      & Total & & & & & N/A & N/A & & & &
      \\ \hline
      \centering 800 & Searching & 3.4 & 3.3 & 3.4 & 3.4 & N/A & N/A & 2.5 & 2.6 & 2.5 & 2.6 \\
      & Planning & 1.2334 & 1.3796 & 1.1835 & 1.1835 & N/A & N/A & 0.9845 & 1.0718 & 0.9845 & 1.0032 \\
      & Total & & & & & N/A & N/A & & & &
      \\ \hline
      
      %%%%%%%%%%%%% end 6th row
    \end{tabular} 
    \begin{flushleft}
    \ \ \ \ \ \ \ \ \ \ \ \ \ \ N/A denotes that the execution did not complete within the limit of 15 min.
    \end{flushleft}

  \end{table*}


==> Table/Table3.tex <==
\begin{table}[tbhp]
  \caption{System settings for field tests}\label{tbl: Algorithm Performance on Sampling Path Planning Approaches}
    \centering
    \begin{tabular}{ | p{3.8cm} || p{1.5cm} |}
      \hline
      \centering
      \textbf{System Configuration} & \textbf{Setting} \\
      \hline \hline
      \centering Average Velocity (m/s) & 0.4 \\
      \centering Sensor (Hz) & 0.1 \\
      \centering GPS Receiver (Hz) & 1 \\
      \centering IMU (Hz) & 1 \\
      \centering ESC (Hz) & 1600 \\
      \centering MCDR of sampling (m) & 3.5 \\ 
      \hline
      %%%%%%%%%%%%% end 6th row
    \end{tabular}
  \end{table}

==> final submitted version/Algorithm/Algorithm1.tex <==
	%\input{Algorithm1}
\SetInd{0.35em}{0.35em}
% \SetAlgoNoLine
\DontPrintSemicolon
\begin{algorithm}[!t]
\small
  \caption{genCoveragePathCycle}\label{alg1}
  \Input{$\hat{A}, d, {\bf{s}}_1\in S$.}
  \Output{$p=({\bf{s}}_1,{\bf{s}}_2,\ldots,{\bf{s}}_\mathcal{N})$.}
  $colACC, rowACC = getACCHexagonalGrid(\hat{A}, d)$\\
  \For {$i = 1:colACC$}
  {
    \For {$j = 1:rowACC$}
    {
      $SLoIs=getCurCellLocation(i,j)$\\
      \eIf {$isCurrentACCFull(SLoIs)$}
      {
        \If {$\sim isNearACCFull($\upshape{`LEFT'}$)$}
          {$p \leftarrow genPath(e_{1,3})$\\
           $flag = \text{True}$\\}
        \eIf {$isNearACCFull($\upshape{`RIGHT'}$)$}
          {$p \leftarrow genPath(e_{2,5},e_{4,6},e_{3,4})$\\}
          {% else
            $p \leftarrow genPath(e_{2,4},e_{3,4})$\\
          }
        \eIf {$isNearACCFull($\upshape{`BOTTOM'}$) \ \& \ isTrue(flag)$}
        { $p \leftarrow genPath(e_{1,7},e_{2,8})$\\
          $p \leftarrow removePath(e_{7,8})$\\
          $flag = \text{False}$\;}
        {% else
          $p \leftarrow genPath(e_{1,2})$\\
        }
        $V = setFineCellVisited(SLoIs)$\\
      }
      { % else
        $U = setFineCellNotVisited(SLoIs)$\\
      }
    }
  }
  \If {$getPathCycleNumber(p)>1$}
  {$p \leftarrow pathSegmentGeneration$($p$)\\
  }
  \Do
  {$~isEmpty(updateCells)$}
  {
    $updateCells = \emptyset$\\
    \ForEach {$ i\in SN$}
    {
      $cells, pattern = findNearCellsInPatterns$($i$)\\
      \If {$\sim isEmpty(cells)$}
      { $updateCells \leftarrow updateCells\cup i$\\
        $p \leftarrow pathSegmentGeneration(p, cells,pattern$)\\
        $SP \leftarrow SP\cup i$\\
        $SN \leftarrow SN\setminus i$\\
      }
    }
  }
\end{algorithm}

==> final submitted version/Algorithm/Algorithm2.tex <==
	%\input{Algorithm2}
	\SetInd{0.35em}{0.35em}
% \SetAlgoNoLine
\DontPrintSemicolon
\begin{algorithm}[!h]
  \caption{coverageSamplingMissionPlanner}\label{alg2}
  \Input{$\hat{A}, e_{bdt}, {\bf{s}}_1\in S$}
  \Output{$p=({\bf{s}}_1, {\bf{s}}_2, ... , {\bf{s}}_\mathcal{N})$}
  $l^*\leftarrow searchOptimalCoverageDensity(\hat{A}, e_{bdt})$\\
  $SLoIs \leftarrow genCoverageSamplingDesign(\hat{A}, l^*)$\\
  $p \leftarrow genCoveragePathCycle(\hat{A}, SLoIs, {\bf{s}}_1)$\\
\end{algorithm}

==> final submitted version/Figures/Fig1.tex <==
\begin{figure}[b!]
    \centering
       \subfigure[]{
    \includegraphics[width=0.22\textwidth]{Figure1.pdf}} \label{fig: sampling_design}
        \subfigure[]{
    \includegraphics[width=0.22\textwidth]{Figure2.pdf}} \label{fig: edge_candidates}
    \caption{(a) Coverage sampling design. The solid red line denotes the study area contour $\hat{A}$. The blue stars denote the SLoIs. (b) Edge candidates and ACC decomposition. The dashed blue lines between the SLoIs denote the edge candidates. The bold black lines denote the ACC contours.}
\end{figure}

==> final submitted version/Figures/Fig10.tex <==
   \begin{figure}[!t]
      \centering
      %\subfigure[]{\label{fig:10}  
      %\includegraphics[width=0.4\textwidth]{Figure10/IMG_2815.JPG}}
            %\subfigure[Aerial photograph of the monitored environment.]{\label{fig:10b}  
      % \includegraphics[width=0.4\textwidth]{Figure10/Pool.png}%}
      
      \includegraphics[width=0.45\textwidth]{Figure10/pool.pdf}
      \caption{Study area and field deployment of the UAV-enabled mobile sensor for water quality monitoring.}
      \label{fig: field deployment}
   \end{figure}

==> final submitted version/Figures/Fig11.tex <==
   \begin{figure*}[!t]
      \centering
      % \subfigure[]{\label{fig:6}
      % \includegraphics[width=0.4\textwidth ]{Figure11/Fig11b.eps}}
      % \subfigure[]{\label{fig:10a}
      % \includegraphics[width=0.4\textwidth]{Figure11/Fig11c.eps}} \\
      % \subfigure[]{\label{fig:6}
      % \includegraphics[width=0.4\textwidth]{Figure11/Fig11d.eps}}
            \subfigure[Generated coverage path for sampling.]{\label{fig:7a}
      \includegraphics[width=0.30\textwidth]{Figure11/path.pdf}}
      		\subfigure[Sampled locations and conductivity map.]{\label{fig:7b}
      \includegraphics[width=0.32\textwidth]{Figure11/Kriging.pdf}}
      		\subfigure[Sampled locations and uncertainty map.]{\label{fig:7c}
      \includegraphics[width=0.32\textwidth]{Figure11/AKV.pdf}}
      \vspace{-5pt}
      \caption{%(a) Generated coverage path for sampling of the proposed method. The solid red and blue contour denote the boundary of the study area and the planned path, respectively. (b) Sampling locations in the field. The blue star markers denote the sampled locations. The black dot markers denote the sampled locations for validation. (c) Temperature mapping result. (d) 
      Field test results using the proposed HGC sampling planner.}
      \label{figurelabel}
   \end{figure*}

==> final submitted version/Figures/Fig2.tex <==
\begin{figure}[h]
	\centering
    \subfigure{
    \includegraphics[height=5.5cm]{Fig2.pdf}}
    \caption{Edge candidates and ACC decomposition. The bold black lines denote the ACC contours. The dashed blue lines between the neibouring SLoIs denote the edge candidates.}
    \label{fig: edge candidates}
\end{figure}

==> final submitted version/Figures/Fig3.tex <==
   \begin{figure}[!h]
      \centering
      \subfigure[Related SLoIs and paths.]{\label{fig:3a}  
      \includegraphics[width=0.20\textwidth]{Fig3a.png}} \
      \subfigure[\textit{V}-modification.]{\label{fig:3b}  
      \includegraphics[width=0.23\textwidth]{Fig3b.png}} \\
      \subfigure[\textit{Z}-modification.]{\label{fig:3c} 
      \includegraphics[width=0.20\textwidth]{Fig3c2.png} \ \ \
      \includegraphics[width=0.22\textwidth]{Fig3c1.png}} \\
      \subfigure[Cycle combination.]{\label{fig:3d}  
      \includegraphics[width=0.35\textwidth]{Fig3d.png}}


          \caption{Strategies of path segment generation.}
          % (a) Path segment generation in an ACC. The current ACC is highlighted by the solid bold contour. The SLoIs of the current and its neighboring ACCs are labeled by their numbers. The dashed blue lines show the possible path segments to be generated. (b) Path cycle combination of two neighboring cycles; (c) Path segment generation for unvisited SLoIs.
      \label{figurelabel}
   \end{figure}
   
   


==> final submitted version/Figures/Fig4.tex <==
   \begin{figure}[!h]
      \centering
      \subfigure[Visiting full ACCs.]{\label{fig:4a}  
      \includegraphics[height=4.2cm]{Fig4a.pdf}} %\ \ \
      \subfigure[Incorporating unvisited SLoIs.]{\label{fig:4b}  
      \includegraphics[height=4.2cm]{Fig4b.pdf}} %\ \ \
	  % \subfigure[]{\label{fig:4c}	   
	  % \includegraphics[height=4.5cm]{Fig4c.pdf}} % \ \ \
\caption{Execution examples of the HGC sampling planner.} %; (c) final coverage path for sampling.}
          % (a) The path segment generation to visit full ACCs. The solid blue lines between APs denote the selected edges as the generated path segments. (b) The generated coverage path after incorporating all unvisited SLoIs. The solid blue lines form the cycle of the planed coverage path. (c) The final coverage path for sampling. The blue star markers denote the distributed sampling locations along the path.
      \label{fig:4}
   \end{figure}


      

   


==> final submitted version/Figures/Fig5.tex <==
\begin{figure}[h!]
      \centering
      \subfigure[RMSE.]{\label{fig:simulation_rmse}  
      \includegraphics[width=0.23\textwidth]{Figure5/RMSE.pdf}} % \ \ \ \ \ \ \ \
      \subfigure[AKV.]{\label{fig:simulation_akv}  
      \includegraphics[width=0.23\textwidth]{Figure5/AKV.pdf}}
      %\subfigure[Ground Truth.]{\label{fig:4a}  
      %\includegraphics[height=4.3cm]{MKVBinary.eps}} 
      %\subfigure[SGSTC.]{\label{fig:4b}  
      %\includegraphics[height=4.3cm]{MKVBruteForce.eps}}

      \caption{Mapping performance on NOMADS dataset.}
      \label{fig:simulation_prediction}
   \end{figure}

==> final submitted version/Figures/Fig6.tex <==
\begin{figure*}[!t]
      \centering
      \subfigure[Ground Truth.]{\label{fig:6a}  
      \includegraphics[width=0.18\textwidth]{Figure6/Fig6_a.png}}
      \subfigure[SGSTC (RMSE).]{\label{fig:6b}  
      \includegraphics[width=0.18\textwidth]{Figure6/Fig6_f.png}}
      \subfigure[DMPP (RMSE).]{\label{fig:6c}  
      \includegraphics[width=0.18\textwidth]{Figure6/Fig6_g.png}}
      %\subfigure[HGTSP.]{\label{fig:4d}  
      %\includegraphics[width=0.18\textwidth]{HGTSPKrigingResult.eps}}
      \subfigure[HGTSP (RMSE).]{\label{fig:6d}  
      \includegraphics[width=0.18\textwidth]{Figure6/Fig6_h.png}}
      \subfigure[HGC (RMSE).]{\label{fig:6e}
      \includegraphics[width=0.18\textwidth]{Figure6/Fig6_j.png}}

      \subfigure[SGSTC (AKV).]{\label{fig:6f}  
      \includegraphics[width=0.18\textwidth]{Figure6/AKVa.jpg}}
      \subfigure[DMPP (AKV).]{\label{fig:6g}  
      \includegraphics[width=0.18\textwidth]{Figure6/AKVb.jpg}}
      \subfigure[HGTSP (AKV).]{\label{fig:6h}  
      \includegraphics[width=0.18\textwidth]{Figure6/AKVc.jpg}}
      \subfigure[HGC (AKV).]{\label{fig:6i}  
      \includegraphics[width=0.18\textwidth]{Figure6/AKVd.jpg}}

\caption{Simulation results of sampling locations and field mapping using different sampling planners (with a budget of 500).} \label{fig:6}
% Energy budget was set at 500. The solid black dots and lines denote the planned SLoIs and sampling paths, respectively. The colors indicate the corresponding predicted value at unobserved locations in the study area.
   \end{figure*} 
   
   
   
   
   

   \begin{comment}

\begin{figure*}[t!]
      \centering
      \begin{tabular}{ccc}
      \adjustbox{valign=b}{\subfigure[Ground truth.\label{subfig-1:dummy}]{%
            \includegraphics[width=.4\linewidth]{GroundTruth.eps}}}
      &      
      \adjustbox{valign=b}{\begin{tabular}{@{}c@{}}
      \subfloat[Square\label{subfig-2:dummy}]{%
            \includegraphics[width=.2\linewidth]{SquareKrigingResult.eps}}
      \subfloat[Hexagonal Random\label{subfig-2:dummy}]{%
            \includegraphics[width=.2\linewidth]{KrigingResult.eps}}
      \end{tabular}}
      \end{tabular}
      \caption{Sampling path planning and mapping results in the simulation. Energy budget is set as 350.}\label{fig:Mapping Results}
    \end{figure*}



   \begin{figure*}[t!]
    \centering
    \begin{tabular}{cc}
    \adjustbox{valign=b}{\begin{tabular}{@{}c@{}}
      \\
    \subfigure[Ground truth.\label{subfig-1:dummy}]{%
          \includegraphics[width=.3\linewidth]{GroundTruth.eps}} 
      \end{tabular}}
    &      
    \adjustbox{valign=b}{\begin{tabular}{@{}c@{}}
    \subfigure[Square\label{subfig-2:dummy}]{%
          \includegraphics[width=.25\linewidth]{KrigingResult.eps}}
    \subfigure[DMPP\label{subfig-2:dummy}]{%
          \includegraphics[width=.25\linewidth]{KrigingResult.eps}}   \\
    \subfigure[TSP\label{subfig-3:dummy}]{%
          \includegraphics[width=.25\linewidth]{KrigingResult.eps}}
     \subfigure[Hexagonal\label{subfig-2:dummy}]{%
          \includegraphics[width=.25\linewidth]{KrigingResult.eps}}
    \end{tabular}}
    \end{tabular}
    \caption{Dummy figure}\label{fig:dummy}
  \end{figure*}       
\end{comment}

==> final submitted version/Figures/Fig7.tex <==
   \begin{figure}[!b]
      \centering
      \includegraphics[height = 5cm]{Figure7/Fig7.eps}
      \caption{Relationships between cell size and number of SLoIs, and total length.} \label{fig:7} 
   \end{figure}

==> final submitted version/Figures/Fig8.tex <==
\begin{figure*}[!t]
    \centering
    % \framebox{\parbox{3.2in}{}}}
          %\subfigure[Searching Time (brute-force).]{\label{fig:8a}  
      %\includegraphics[height = 4.8cm]{Figure8/Fig8_a.eps}} \ \
        %        \subfigure[Planning Time (brute-force).]{\label{fig:8b}  
      %\includegraphics[height = 4.8cm]{Figure8/Fig8_b.eps}} \ \
                %\subfigure[Total Time (brute-force).]{\label{fig:8c}  
      %\includegraphics[height = 4.8cm]{Figure8/Fig8_c.eps}} \\
         %\ \
                \subfigure[Searching Time (binary).]{\label{fig:8d}  
      \includegraphics[height = 4.8cm]{Figure8/Fig8_d.eps}} \ \
                      \subfigure[Planning Time (binary).]{\label{fig:8e}  
      \includegraphics[height = 4.8cm]{Figure8/Fig8_e.eps}} \ \
                      \subfigure[Total Time (binary).]{\label{fig:8f}  
      \includegraphics[height = 4.8cm]{Figure8/Fig8_f.eps}} \ \
    
  \caption{Algorithm performance related to computational efficiency.}
  \label{fig:8}
  \end{figure*} 

==> final submitted version/Table/Table1.tex <==
\begin{table}[h!]
	\renewcommand{\arraystretch}{1.05}
    \caption{Mapping performance on NOMADS dataset.} \label{tab:1}
    \centering
\begin{tabular}{ | p{0.8cm} | b{0.9cm} || p{0.9cm} | p{0.9cm} | p{0.9cm} | p{0.8cm} |}
      \hline
      \centering
      \textbf{Budget} & \centering \textbf{Metric} & \textbf{SGSTC } & \textbf{DMPP } & \textbf{HGTSP} & \textbf{HGC}
      \\
      \hline\hline
      \centering & \centering $l^*$ & 5.36 & 5.52 & 4.74 & 4.58 \\
      \centering 400 & \vspace{-2pt} \centering $e_{RMS}$ \vspace{0.1bp} & 2.8272 & 2.2149 & \cellcolor[gray]{.8} 1.7870 & 1.7960 \\
      & \centering $\bar{\Sigma}_{K}$ & 1.2134 & 1.3072 & 1.3704 & \cellcolor[gray]{.8} 0.7662
      \\ \hline
      \centering & \centering $l^*$ & 4.51 & 4.84 & 3.78 & 3.68  \\
      \centering 500 & \vspace{-2pt} \centering $e_{RMS}$ \vspace{0.1bp} & 2.5179 & 1.9065 & 2.1930 & \cellcolor[gray]{.8} 1.4064 \\
      & \centering $\bar{\Sigma}_{K}$ & 1.2907 & 1.6925 & 1.9507 & \cellcolor[gray]{.8} 0.9302
      \\ \hline
      \centering & \centering $l^*$ & 4.05 & 4.16 & 3.10 & 3.10 \\
      \centering 600 & \vspace{-2pt} \centering $e_{RMS}$ \vspace{0.1bp} & 1.9496 & 1.4642 & \cellcolor[gray]{.8} 1.1765 & \cellcolor[gray]{.8} 1.1765 \\
      & \centering $\bar{\Sigma}_{K}$ & 2.3832 & 1.2136 & \cellcolor[gray]{.8} 0.5967 & \cellcolor[gray]{.8} 0.5967
      \\ \hline
      \centering & \centering $l^*$ & 3.76 & 3.68 & N/A & 2.91 \\
      \centering 700 & \vspace{-2pt} \centering $e_{RMS}$ \vspace{0.1bp} & 1.6517 & 1.4064 & N/A & \cellcolor[gray]{.8} 1.1358 \\
      & \centering $\bar{\Sigma}_{K}$ & 0.8850 & 1.0521 & N/A & \cellcolor[gray]{.8} 0.2921
      \\ \hline
      \centering & \centering $l^*$ & 3.25 & 3.35 & N/A & 2.51 \\
      \centering 800 & \vspace{-2pt} \centering $e_{RMS}$ \vspace{0.1bp} & 1.7153 & 1.6199 & N/A & \cellcolor[gray]{.8} 0.9214 \\
      & \centering $\bar{\Sigma}_{K}$ & 0.7389 & 0.6521 & N/A & \cellcolor[gray]{.8} 0.4666
      \\ \hline
    \end{tabular} 
    \begin{flushleft}
    \ \ \ \ \ N/A: Execution did not complete within the time limit of 15 min.
	\\
	\ \ \ \ \ Grey color highlights the best prediction results.    
    \end{flushleft}

  \end{table}


==> final submitted version/Table/Table2-backup.tex <==
\begin{table}[htbp]
  \caption{Algorithm Performance on Computational Efficiency}\label{tbl: Algorithm Performance on Sampling Path Planning Approaches}
    \centering
    \begin{tabular}{ | p{0.9cm} | p{1.5cm} || p{1.1cm} | p{1cm} | p{1.1cm} | }
      \hline
      \textbf{Energy Budget} & \centering \textbf{Algorithm} & \textbf{Searching Time } & \textbf{Planning Time } & \textbf{Total Time }\\
      (km) & & (s) & (s) & (s)  \\
      \hline \hline
      & \text{SGSTC} & 39.47 & 0.98 & 40.45
      \\
      & \text{DMPP} & 106.50 & 0.71 & 107.21
      \\
      \centering 250 & \text{RSTSP} & 4277.41 & 2.85 & 4280.26
      \\
      & \text{HGSTC} & 34.75 & 0.77 & 35.52
      \\
      & \text{HGC} & 34.87 & 0.24 & \cellcolor[gray]{.8} 35.11
      \\
      & \text{HGC (binary)} & 2.59 & 0.27 & 2.86
      \\ \hline \hline
      & \text{SGSTC} & 40.09 & 1.05 & 41.14
      \\
      & \text{DMPP} & 116.27 & 0.77 & 117.04
      \\
      \centering 350 & \text{RSTSP} & 4278.55  & 3.09 & 4281.64
      \\
      & \text{HGSTC} & 35.73 & 0.79 & 36.52
      \\
      & \text{HGC} & 34.88 & 0.29 & \cellcolor[gray]{.8} 35.17 
      \\
      & \text{HGC (binary)} & 1.89 & 0.31 & 2.20
      \\ \hline \hline
      & \text{SGSTC} & 39.68 & 1.23 & 40.91
      \\
      & \text{DMPP} & 120.84 & 1.06 & 121.97
      \\
      \centering 450 & \text{RSTSP} & 4282.62 & 4.18 & 4286.80
      \\
      & \text{HGSTC} & 35.26 & 1.05 & 36.31
      \\
      & \text{HGC} & 35.69 & 0.38 & \cellcolor[gray]{.8} 36.07
      \\
      & \text{HGC (binary)} & 2.64 & 0.37 & 3.01
      \\ \hline
      %%%%%%%%%%%%% end 6th row
    \end{tabular}
  \end{table}


==> final submitted version/Table/Table2.tex <==
\begin{table*}[t!]
  \caption{Algorithm Performance on Computational Efficiency}\label{tbl: Algorithm Performance on Sampling Path Planning Approaches}
    \centering
    \begin{tabular}{ | p{1cm} | p{1.1cm} || p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} | p{1cm} |}
      \hline
      \centering
      \textbf{Energy Budget} & \centering \textbf{Processing Time} & \multicolumn{2}{c|}{\textbf{SGSTC}} & \multicolumn{2}{c|}{\textbf{DMPP}} & \multicolumn{2}{c|}{\textbf{HGTSP}} & \multicolumn{2}{c|}{\textbf{HGSP}} & \multicolumn{2}{c|}{\textbf{HGC}}
      \\
      \hline
      \centering
      $b$ (km) & (s) & Brute-force & Binary &  Brute-force & Binary &  Brute-force & Binary & Brute-force & Binary & Brute-force & Binary \\ \hline \hline
      \centering 400 & Searching & 1.36 & 6.5 & 5.5 & 5.7 & N/A & 4.8 & 4.6 & 4.8 & 4.6 & 4.8 \\
      & Planning & 0.82 & 1.7330 & 2.0412 & 2.5893 & N/A & 1.5776 & 1.8274 & 1.6062 & 1.8274 & 1.6062 \\
      & Total & 2.18 & & & & N/A & & & & &
      \\ \hline
      \centering 500 & Searching & 4.5 & 4.5 & 4.7 & 4.9 & N/A & 3.7 & 3.7 & 3.7 & 3.7 & 3.7 \\
      & Planning & 2.4891 & 2.4891 & 1.8367 & 1.8225 & N/A & 1.4626 & 1.4626 & 1.4626 & 1.4626 & 1.4626 \\
      & Total & & & & & N/A & & & & &
      \\ \hline
      \centering 600 & Searching & 3.8 & 4.1 & 4.2 & 4.3 & N/A & 3.1 & 3.1 & 3.2 & 3.1 & 3.2 \\
      & Planning & 1.4565 & 2.0527 & 1.9664 & 1.6368 & N/A & 1.2319 & 1.2319 & 1.2548 & 1.2319 & 1.2548 \\
      & Total & & & & & N/A & & & & &
      \\ \hline
      \centering 700 & Searching & 3.6 & 3.8 & 3.7 & 3.7 & N/A & N/A & 2.9 & 3 & 2.9 & 3 \\
      & Planning & 1.3357 & 1.4565 & 1.4757 & 1.4757 & N/A & N/A & 1.2120 & 1.2448 & 1.2120 & 1.2448 \\
      & Total & & & & & N/A & N/A & & & &
      \\ \hline
      \centering 800 & Searching & 3.4 & 3.3 & 3.4 & 3.4 & N/A & N/A & 2.5 & 2.6 & 2.5 & 2.6 \\
      & Planning & 1.2334 & 1.3796 & 1.1835 & 1.1835 & N/A & N/A & 0.9845 & 1.0718 & 0.9845 & 1.0032 \\
      & Total & & & & & N/A & N/A & & & &
      \\ \hline
      
      %%%%%%%%%%%%% end 6th row
    \end{tabular} 
    \begin{flushleft}
    \ \ \ \ \ \ \ \ \ \ \ \ \ \ N/A denotes that the execution did not complete within the limit of 15 min.
    \end{flushleft}

  \end{table*}


==> final submitted version/Table/Table3.tex <==
\begin{table}[tbhp]
  \caption{System settings for field tests}\label{tbl: Algorithm Performance on Sampling Path Planning Approaches}
    \centering
    \begin{tabular}{ | p{3.8cm} || p{1.5cm} |}
      \hline
      \centering
      \textbf{System Configuration} & \textbf{Setting} \\
      \hline \hline
      \centering Average Velocity (m/s) & 0.4 \\
      \centering Sensor (Hz) & 0.1 \\
      \centering GPS Receiver (Hz) & 1 \\
      \centering IMU (Hz) & 1 \\
      \centering ESC (Hz) & 1600 \\
      \centering MCDR of sampling (m) & 3.5 \\ 
      \hline
      %%%%%%%%%%%%% end 6th row
    \end{tabular}
  \end{table}

==> final submitted version/Table/Table4.tex <==
\begin{comment}
\begin{figure*}[!t]
  %\vspace*{\floatsep} 
  \begin{minipage}{.4\linewidth}
%\begin{table}[!t]
    \centering
    \captionof{table}{Algorithm Performance of Field Tests}\label{tbl: Algorithm Performance on Sampling Path Planning Approaches}
    \begin{tabular}{ | p{1cm} || p{1cm} | p{1cm} | p{1cm} | p{0.9cm} |}
      \hline
      \centering
      \textbf{Metric} & \textbf{SGSTC} & \textbf{DMPP} & \textbf{RSTSP} & \textbf{HGC} \\
      \hline \hline
      \centering \text{RMSE} & \small 0.1545 & \small 0.1429 & \small 0.1282 & \cellcolor[gray]{.8} \small 0.1277 \\ %\cellcolor[gray]{.8} 0.1277
      \hline
      \centering \text{AKV} & \small 0.1545 & \small 0.1429 & \small 0.1282 & \cellcolor[gray]{.8} \small 0.1277 \\
      \hline
      %%%%%%%%%%%%% end 6th row
    \end{tabular}
  %\end{table}
  \end{minipage}%
  \begin{minipage}{0.6\linewidth}
        \subfigure[RMSE.]{\label{fig:6d}  
    \centering \includegraphics[width=0.5\textwidth]{Figure11/Fig11e.eps}}
            \subfigure[AKV.]{\label{fig:6d}  
    \centering \includegraphics[width=0.5\textwidth]{Figure11/Fig11e.eps}}
    \captionof{figure}{Filed mapping results of the proposed HGC sampling planner.}
  \end{minipage}
\end{figure*}%
 \end{comment}


\begin{table}[!t]
  \renewcommand{\arraystretch}{1.2}
  \caption{Planner performance of field tests.}\label{tbl: Algorithm Performance on Sampling Path Planning Approaches}
    \centering
    \begin{tabular}{ | p{1cm} || p{0.9cm} | p{0.8cm} | p{0.9cm} | p{0.8cm} |}
      \hline
      \centering
      \textbf{Metric} & \textbf{SGSTC} & \textbf{DMPP} & \textbf{HGTSP} & \textbf{HGC} \\
      \hline \hline
      \centering $e_{RMS}$ \vspace{0.1bp} & 2.5155 & 1.0760 & 0.6821 & \cellcolor[gray]{.8} 0.6754 \\ %\cellcolor[gray]{.8} 0.1277
      \hline
	  \centering $\bar\Sigma_K$ & 1.4196 & 0.8083 & 0.1961 & \cellcolor[gray]{.8} 0.1072 \\
      \hline
      %%%%%%%%%%%%% end 6th row
    \end{tabular}
  \end{table}


